PowerNet: Transferable Dynamic IR Drop Estimation via Maximum Convolutional Neural Network

IR drop is a fundamental constraint required by almost all chip designs. However, its evaluation usually takes a long time that hinders mitigation techniques for fixing its violations. In this work, we develop a fast dynamic IR drop estimation technique, named PowerNet, based on a convolutional neural network (CNN). It can handle both vector-based and vectorless IR analyses. Moreover, the proposed CNN model is general and transferable to different designs. This is in contrast to most existing machine learning (ML) approaches, where a model is applicable only to a specific design. Experimental results show that PowerNet outperforms the latest ML method by 9% in accuracy for the challenging case of vectorless IR drop and achieves a 30 times speedup compared to an accurate IR drop commercial tool. Further, a mitigation tool guided by PowerNet reduces IR drop hotspots by 26% and 31% on two industrial designs, respectively, with very limited modification on their power grids.

==> _txt/1_background.tex <==
\section{Background}

\subsection{IR Drop Problem}

\begin{figure}[!bth]
  \centering
  \begin{minipage}[t]{3in}
    \includegraphics[width=3in]{resist-min.pdf}
  \caption{Resistance distribution.}
  \label{resist}
  \end{minipage}
\end{figure}

According to Ohms Law, excessive IR drop can be caused by either high current or high resistance. Because designs in our experiments all adopt a uniform power delivery network (PDN), the resistance distribution across the whole design is also rather uniform. Figure \ref{resist} shows an example. The maximum discrepancy in resistance across design is only around $(470-430)/450 = 9\%$ of averaged resistance. Thus in PowerNet, we choose not to spend extra time calculating resistance for each cell. For designs with non-uniform PDN, each cell's power value can be scaled by its resistance. When resistance is considered consistent, current becomes the only key issue in IR drop estimation. Since local power consumption is proportional to local current, PowerNet utilizes cell power as input features.

However, IR drop for each cell will not simply be proportional to its own power because of both spatial and time reasons. Spatially, local current is proportional to the sum of power demand of all cells in a local region. That means power of neighboring cells also contributes to IR drop of the analyzed cell. It motivates us to adopt CNN in PowerNet, which is inherently designed for learning scalable two-dimensional patterns. Besides, a region with high overall power demand may still not be IR drop hotspot. Because cells in this region may not switch at the same time, depending on when the signal arrives. Such asynchronous switching disperses voltage drop into a larger timing window. As a result, IR drop, the highest transient voltage drop, can remain to be low. PowerNet uses time-decomposed power and maximum structure to measure such influence.



